Rethinking the Event Coding Pipeline with Prompt Entailment

For monitoring crises, political events are extracted from the news. The large amount of unstructured full-text event descriptions makes a case-by-case analysis unmanageable, particularly for low-resource humanitarian aid organizations. This creates a demand to classify events into event types, a task referred to as event coding. Typically, domain experts craft an event type ontology, annotators label a large dataset and technical experts develop a supervised coding system. In this work, we propose PR-ENT, a new event coding approach that is more flexible and resource-efficient, while maintaining competitive accuracy: first, we extend an event description such as "Military injured two civilians'' by a template, e.g. "People were [Z]" and prompt a pre-trained (cloze) language model to fill the slot Z. Second, we select answer candidates Z* = {"injured'', "hurt"...} by treating the event description as premise and the filled templates as hypothesis in a textual entailment task. This allows domain experts to draft the codebook directly as labeled prompts and interpretable answer candidates. This human-in-the-loop process is guided by our interactive codebook design tool. We evaluate PR-ENT in several robustness checks: perturbing the event description and prompt template, restricting the vocabulary and removing contextual information.

==> archive.tex <==
Let $C$ be the number of intensity classes in our scale. We build the following generative model:
\begin{align}
    \iota_t &\sim \categorical \left(\{1, \ldots, C\}\right) \\
    f_t \mid \iota_t &\sim \poisson(\lambda_{\iota_t}) \\
    g_t \mid \iota_t &\sim \gaussian(\mu_{\iota_t}, \sigma^2 I) \\
    % \langle v, a \rangle \mid \iota_t &\sim \NN{\iota_t}
    \langle v, a \rangle \mid \iota_t &\sim \text{BagOfWords}
\end{align}

We additionally want two things:
First, we want to impose the constraint that, on average, a higher intensity event is more likely to cause greater fatalities.
Second, we would like higher intensity events to be assigned a higher Goldstein value.
We describe how this is achieved further down below.


The generative story is this: We sample a discrete, ordinal latent variable $\iota$ describing the intensity of the event. In this scale, the maximum intensity is $C$, and the minimum intensity is one.\footnote{This is analogous to the Richter scale, used to describe the magnitude of earthquakes.}
Conditioned on the intensity, we sample the number of fatalities $f$ associated with the event, the Goldstein value of the event, and the predicate-argument structures $\langle v, a \rangle$ of the event's textual description. Generally speaking, the specific choice of these three variables is not important; our formulation is able to take any set of correlates and create a discretized, interpretable, and ordinal scale directly from data.

\paragraph{Priors.} Define $\lambda_0 = 1$.
Sample $\Delta_i \sim \gam(\gamma, 1)$ where $c \in \{1, \ldots, C\}$.
The $\Delta_i$ is understood to be the log difference between the $\lambda_i$, i.e. $\Delta_i = \log \lambda_i - \log \lambda_{i-1}$.
Then, define $\lambda_i = \exp\left(\sum_{c=1}^i \Delta_c\right)$
As an example, this yields $\lambda_2 = \exp\left(\log \lambda_2 - \log \lambda_1 + \log \lambda_1 - \log \lambda_0\right)$,

See \url{https://math.stackexchange.com/questions/250059/sum-of-independent-gamma-distributions-is-a-gamma-distribution}

\begin{align}
    y_i &\sim \textrm{Pois}(\lambda_{z_i}) \\
    z_i &\sim \textrm{Cat}(\pi_1,\dots,\pi_C)\\
    \{\lambda_1,\dots,\lambda_C\} &\sim \textrm{OrderedPrior}(\dots)
\end{align}

where $\lambda_c \geq \lambda_{c+1}$.


\section{Evaluation}

At test-time, we do not have access to the fatality counts. We do posterior inference to obtain them. If our model is good, then it should be able to handle this well.

